OpenBias: Open-set Bias Detection in Text-to-Image Generative Models

Text-to-image generative models are becoming increasingly popular and accessible to the general public. As these models see large-scale deployments, it is necessary to deeply investigate their safety and fairness to not disseminate and perpetuate any kind of biases. However, existing works focus on detecting closed sets of biases defined a priori, limiting the studies to well-known concepts. In this paper, we tackle the challenge of open-set bias detection in text-to-image generative models presenting OpenBias, a new pipeline that identifies and quantifies the severity of biases agnostically, without access to any precompiled set. OpenBias has three stages. In the first phase, we leverage a Large Language Model (LLM) to propose biases given a set of captions. Secondly, the target generative model produces images using the same set of captions. Lastly, a Vision Question Answering model recognizes the presence and extent of the previously proposed biases. We study the behavior of Stable Diffusion 1.5, 2, and XL emphasizing new biases, never investigated before. Via quantitative experiments, we demonstrate that OpenBias agrees with current closed-set bias detection methods and human judgement.

==> sec/3_method.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/method/Method_overview.pdf}
    \caption{Method.}
    \label{fig:method}
\end{figure*}

\section{Method}
In this section, we present OpenBias, our pipeline for proposing, assessing, and quantifying biases in text-to-image generative models. %without relying on a predefined list. 
We present an overview of our framework in \cref{fig:method}. 
% We start from a dataset of real captions and we build, leveraging a LLM, a knowledge base of biases composed of specific information such as captions, questions, and classes all associated with the bias. This process allows us to create domain-specific knowledge, which may vary based on the dataset.
Starting from a dataset of real textual captions, we leverage a Large Language Model (LLM) to build a knowledge base of possible biases present in the dataset. This process enables the identification of domain-specific biases, % which were previously 
unexplored up to now.  In the second stage, % of our pipeline, 
we synthesize images using the target generative model, conditioned on captions where a potential bias has been identified.  %the assigned captions for a particular bias are used to synthesize bias-specific images leveraging the target generative model. 
% After generating the images, we leverage the knowledge base to assess and quantify the presence of each bias via Vision Question Answering (VQA) applied to the generated images. 
Lastly, we propose to assess the biases with a VQA model; this involves querying the model with caption-specific questions extracted during the bias proposal phase.

\subsection{Bias Proposals}
\label{sec:bias_proposal}
%In this section, we explain our \textit{bias proposals} procedure able to build the knowledge base $\knowledgebase$ of biases required to recognize and quantify them. This procedure leverages in-context learning, a well-known technique that consists of assigning to an LLM a specific task during inference, accompanied by specific instructions on how to perform it. In addition, a set of examples is given to the model to improve its performance similarly to existing works~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. Please see the supplementary material for further details about the system task and examples given to the LLM.
%We start from a set of captions $\datasetcaptions$ provided by a real dataset. The LLM is explicitly tasked to provide knowledge about biases that may occur during the generation process if the specific captions are given to a generative model, thereby preventing the LLM from extracting biases inherent in the caption. Given a caption, we ask the LLM to output three main pieces of information: the bias name, a set of classes, and a question. The name allows us to identify the bias under study, and the set of classes and questions, allow us to recognize and quantify the bias at the third stage of our pipeline. To give a concrete example, if the caption is \textit{"A person running"} one of the proposed biases may be \textit{"person gender"}. In this case, the other pieces of information for this bias may be \textit{"Male"} and \textit{"Female"} as classes and \textit{"What is the gender of the person in the picture?"} as the question. 

%In this section, we detail our \emph{bias proposal} procedure. 
Given a dataset of real captions $\datasetcaptions$, we construct a knowledge base $\knowledgebase$ of possible biases. For each caption in the dataset, we task a LLM with providing three outputs: the potential bias name, a set of classes associated with the bias, and a question to identify the bias. %In practice, if the caption is \textit{"A person running"} one of the proposed biases may be \textit{"person gender"}. In this case, the other pieces of information for this bias may be \textit{"Male"} and \textit{"Female"} as classes and \textit{"What is the gender of the person in the picture?"} as the question. 


More formally, given a caption $\singlecaption \in \datasetcaptions$, let us denote the LLM's output as a set of triplets $\mathtt{LLM}( \singlecaption)=
\{(\biasname^t_i, \mathcal{C}^t_i, q^t_i)\}_{i=1}^{n_t}$ %, \cdots, (\biasname^t_M(t), \mathcal{C}^t_{M(t)}, q^t_{M(t)}) \}$,
% \begin{equation}
%     \label{eq:llm}
%     \text{LLM}( \singlecaption)=\left\{\biasname, \hat{\mathcal{C}}, \hat{q}_t \right\}
% \end{equation}
where the cardinality $n_t$ of the set is caption dependent, and each triplet $(\biasname, \mathcal{C}, q)$ has a proposed bias $\biasname$, % the proposed bias name, 
 the set of associated classes $\mathcal{C}$, and $q$ the question assigned to the specific caption and bias $\singlecaption$. %Note that the number of triplets $M$ varies and depends on the captions. 
 To obtain this set, we propose to use in-context learning \cite{NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}, providing task description and demonstrations directly in the textual prompt.\footnote{We refer the reader to {\supp} for details regarding the prompt formulation.} 

Next, we build the knowledge base $\knowledgebase$ by aggregating the per-caption information on the whole dataset. Specifically, we group the captions based on the bias name and the associated classes, yielding: 
%We analyze in detail this post-processing procedure in the supplementary material. Thus, given a bias $\bias$, we define its knowledge base as:
\begin{equation}
    \label{eq:knowlegebase}
    \mathcal{B}_j = (\Tj, \classes, \mathcal{Q}_j), \quad \mathcal{B}_j \in \knowledgebase
    %\defineKB
\end{equation}
where $\Tj \subseteq \datasetcaptions$ is the set of captions, $\setquestions$ is the set of related questions, and $\classes$ as set of classes associated to the bias $\bias$. 

%We denote a piece of specific information as $\hat{\cdot}$ when entirely generated by the LLM. 
%The information from the set of classes $\classes$ and $\setquestions$ will be used, in the third phase, as input to the VQA as a closed-form question to recognize the specific bias in the generated images. Executing this procedure on a set of captions builds a knowledge base of biases with specific information required to recognize them effectively.
% The above-explained procedure can lead to undesirable consequences when a specific, bias-related characteristic is defined in the caption. For example, a sentence of the type \textit{"A man running"} should be avoided while studying gender-related biases as it explicitly specifies the attribute of the bias under study. To avoid this outcome, we apply a two-stage filtering: first, we ask the LLM to output whether the answer to the question $\singlequestion$ is embedded in the caption itself, if so the caption will not be considered for the specific bias $\bias$. Secondly, we leverage ConceptNET \cite{ConceptNET} to extract synonyms of the classes $\classes$ for the specific bias $\bias$, then we filter the captions containing such synonyms. The first stage is required since LLM knows the context of the caption, and synonyms may not capture the whole picture. On the other hand, the second stage ensures that specific words related to the bias are not present in the caption improving the robustness of the pipeline.

However, as discussed in \Cref{sec:intro}, we are interested in studying the tendency of the model to generate a specific class when it is not explicitly described in the caption. To address this, we implement a two-stage filtering procedure. First, we ask the LLM to output whether the answer to the question $\singlequestion$ is explicitly present in the caption $\singlecaption$. Secondly, we leverage ConceptNET \cite{ConceptNET} to identify synonyms for the classes $\classes$ related to the specific bias $\bias$, and filter out the captions containing these synonyms. We empirically observe that the combination of these two stages produces more robust results. %We refer the reader to the {\supp} for details regarding the system prompts we use for the LLM.

By executing the aforementioned steps, we generate bias proposals in an open-set manner tailored to the given dataset. In the following sections, we elaborate on the process of assessing and quantifying bias in a target generative model.

\subsection{Bias Assessment and Quantification}
%At this stage, we aim to assess the presence of each previously proposed bias. We employ the target generative model G to produce a synthetic dataset using the set of captions $\Tj \subseteq \datasetcaptions$ associated with the bias $\bias$. This process results in a set of images for each bias. The assessment of biases is conducted via Vision Question Answering. For each bias $\bias$, we utilize a state-of-the-art VQA model on the generated images, answering the associated questions $\setquestions$ in a closed form by providing the model with answer choices resembling the classes $\classes$. This approach enables statistical analyses by exploring the distribution over the classes. During this phase, we consider the context of each caption by building the generated dataset with $N$ images for every caption. This consideration of context is essential for comprehensive bias evaluation. This framework provides the basis for studying the bias in a contextualized or context-free form.

Let $\generator$ be the text-to-image generative model that we aim to evaluate. Our objective is to assess the presence of the biases identified in the previous steps within the images synthesized by the model. 
For each bias $\bias \in \knowledgebase$, we generate a set of images for each relevant caption $\mathcal{I}(\bias) = \{\mathcal{I}_{t}\}, \forall t \in \Tj$, with $\mathcal{I}_{t}=\{I_t^k = \generator(t)\}_{k=1}^N$. In this stage, we use $N$ different random seeds for each single caption $t$ to obtain a distribution of the model's output on the same prompt. 
To assess the bias, we propose to leverage a state-of-the-art Vision Question Answering (VQA) model. The VQA processes the images $\mathcal{I}(\bias)$ along with their associated questions from the set $\setquestions$, and is tasked with choosing from the possible classes $\classes$. Formally, we denote the predicted class as 

\begin{equation}
    \label{eq:vqa}
    \hat{c} = \text{VQA}(I_t^k, q_j, \mathcal{C}_j)
\end{equation}

This process allows us to gather statistics on the distribution of the classes on a set of images, and employ them to quantify the severity of the bias. 

Furthermore, we investigate two distinct scenarios, namely \emph{context-aware}, where we analyze the bias on caption-specific images $\mathcal{I}_{t}$, and \emph{context-free}, where we consider the whole set of images associated to one bias $\mathcal{I}(\bias)$. Next, we describe the difference between the two.

\subsubsection{Context-Aware Bias}
\label{sec:context_aware}
% In the contextualized formulation, we are interested in capturing the bias $\bias$ considering the context of the caption. For instance, let's suppose we possess two captions of the form \textit{``A military person is running"} and \textit{``A person is running"}, they are both agnostic to the bias \textit{``person gender"}, but the bias direction and magnitude may vary depending on the context, thus, to take the context into account we generate $N$ images for each caption $\singlecaption \in \Tj$. We define this set of images as $\defineI$ and the expected probability over the classes $\classes$ condition on context $t$ as:
% $$
%     \definePcontext
% $$
% where: $\indicatorfunction$ denotes the indicator function that is $1$ when $c$ is equal to the output of the $VQA$ model applied to the generated image $I_z$, and $0$ otherwise and $\hat{q}_t$ is the question assigned to $t$ from the previous phase. This formulation allows us to study how the bias $\bias$ varies in relation to the context of each caption $t$.

As discussed in \Cref{sec:intro}, our focus lies in examining bias exclusively when the classes are not explicitly mentioned in the caption. The bias proposals pipeline described in \cref{sec:bias_proposal} filters out such cases; nevertheless, there could be additional aspects within the caption that impact the final outcome. For example, the two captions \textit{``A military is running"} and \textit{``A person is running"} are both agnostic to the bias \textit{``person gender"}, but the direction and magnitude of the bias may be very different in the two cases. 
To consider the role of the context in the bias assessment, we collect statistics at the caption level, analyzing the set of images $\mathcal{I}_t$ produced from a specific caption $t \in \Tj$. In practice, we compute the probability of each class as:

\begin{equation}
    \label{eq:context_aware}
    p(c_i | t, \bias) = \dfrac{1}{N} \sum_{k=1}^N \indicatorfunction \bigl(\hat{c}=c_i \bigr)
\end{equation}

with $c_i \in \classes$, $\hat{c} = \text{VQA}(I_t^k, q_j, \classes)$ the prediction of the VQA as defined in \cref{eq:vqa}, and $\indicatorfunction(\cdot)$ the indicator function.

\subsubsection{Context-Free Bias}
% In this approach, we are interested in understanding the behavior of the target generative model without considering the context. This is significant as it allows us to study the scale of the impact of context on the given bias and facilitates the study of the model in a more general setting. Concretely, given a bias $\bias$, we define its synthetic dataset as $\definesyntheticdataset$, that is we consider the whole dataset of generated images regardless of the caption context. In this scenario, we compute the context-free expected probability distribution over the classes $\classes$ as:
% $$
%     \definePfreecontext
% $$

Differently from the context-aware scenario, our interest lies in characterizing the overall behavior of the model $\generator$. This is crucial as it offers valuable insights into aspects such as the majority class (\ie the direction toward which the bias tends) and the overall intensity of the bias. To effectively exclude the role of the context in the captions, we propose to average over all the possible captions $t \in \Tj$ related to that bias $\bias$:

\begin{equation}
    \label{eq:context_free}
    p(c_i | \bias) = \dfrac{1}{|\Tj|} \sum_{t \in \Tj} P(c_i|t, \bias),
\end{equation}

where the probability of the right-hand side is computed with \cref{eq:context_aware}.

\subsubsection{Bias Quantification and Ranking}
% The open-set nature of our setting challenges the study and understanding of the multiple biases. We address this issue by ranking the biases based on their intensity. We use the entropy computed over the categorical distributions defined above. Since we are required to compare these values across different distributions, we use the normalized entropy $\mathcal{H}$ \cite{wilcox1967indices}. In order to make the entropy more human-readable we define the intensity of a bias $\bias$ as $1-\mathcal{H}$. The intensity is bounded in $[0,1]$ where $0$ describes high uncertainty over the classes and thus low bias, instead $1$ expresses low uncertainty thus high bias. We apply this formulation over the contextualized bias and context-free bias defined above. When applied to the contextualized distribution we average over all the captions $\Tj$. This formulation allows us to rank the found biases by bias intensity.

Following existing work \cite{fairDiffusion2023, xu2018fairgan}, we adopt the definition of fairness outlined in \cref{eq:bias_eq}. We consider the model $\generator$ as unbiased with respect to a concept $\bias$ when the distribution of the possible classes $c_i \in \classes$ is uniform. 
To quantitatively assess the severity of the bias, we compute the entropy of the probability distribution of the classes obtained using either \cref{eq:context_aware} or \cref{eq:context_free}. In order to compare biases with different numbers of classes, we normalize the entropy by the maximum possible entropy \cite{wilcox1967indices}. Additionally, we adjust the score for enhanced human readability. In practice, our bias severity score is defined as follows: \elia{$p(c | Bj)$ is not defined before...}

\begin{equation}
    \label{eq:entropy_score}
    \bar{\mathcal{H}}(\bias) = 1 - \dfrac{\mathbb{E}[-\log p(\classes | \bias)]}{\log(|\classes|)} 
\end{equation}

The resulting score is always bounded $\bar{\mathcal{H}}(\bias) \in [0,1]$. Lower values indicate an unbiased concept, while scores close to one signify a biased concept.
% In addition, a set of examples is given to the model to improve its performance similarly to existing works~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. We ask the LLM to output a set of biases for each caption alongside a set of classes and a question for each identified bias. By doing so we build a knowledge base of biases which are specific for each caption, comprising a set of classes and questions. Afterward, we sample $N$ captions for each bias and we generate $K$ images for each caption, in this way we make sure that if the bias is present it does not depend from the caption. This process generates $N\times K$ images for each bias. The third and final stage exploits a Vision Question Answering model which is applied to the generated images and, for each bias, we ask the model to answer the bias specific question given by the LLM in a closed form by providing the classes. We quantify the presence of the biases by applying two metrics to the extracted class distributions: Entropy and KL divergence. 


% To be added in the method section:

% We first perform in-context learning on a LLM which is a well-known zero-shot method. In-context learning assigns to the LLM a specific task during inference, accompanied by specific instructions on how to perform it, and, in addition, a set of examples is given to the model to improve its performance~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. 
% Our pipeline is composed of three main stages: bias identification, image generation and bias recognition. In the first stage, we task a LLM to identify a set of possible biases that may occur during the generation process given a set of captions. By doing so we identify the set of biases that are going to be studied 
% In our pipeline, we make use of in-context learning. This method assigns to the LLM a specific task during inference, accompanied by specific instructions on how to perform it, and, in addition, a set of examples is given to the model to improve its performance~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}.

% we exploit the recent advancements in foundation models~\cite{NEURIPS2020_gpt_3_few_shot, NEURIPS2022_Chain_of_Thougth, li2023blip2, liu2023llava, liu2023improvedllava}. 

==> sec/6_evaluation.tex <==
\section{Evaluation}

\input{tables/LLM_eval}
The open-set nature of our setting challenges the zero-shot performance of each pipeline component, consequently, it is crucial to evaluate each module. We evaluate the LLM with a classification task on two datasets: StereoSet~\cite{nadeem2020stereoset} and Crows~\cite{nangia2020crows}. StereoSet~\cite{nadeem2020stereoset} is composed of $3707$ sentences spanning gender, race, religion, and profession as classes. Crows~\cite{nangia2020crows} comprises $2637$ sentences with the same classes as StereoSet with the addition of sexual orientation, age, nationality, disability, and physical appearance. We task the LLM to detect these stereotypes within the sentences. The results of these experiments are shown in table~\ref{tab:LLM_eval}. The performance of the language mode appears satisfactory for identifying stereotypes. This evaluation serves as a proxy for evaluating our bias proposal module, in our setting we ask the language model to generate a set of biases (proposals) based on a given caption. Therefore, our primary interest lies in evaluating the model's proposals, specifically its top-k performance. 

\input{tables/KL_div_fairface_eval}
We ablate the VQA module showing its agreement with FairFace~\cite{Karkkainen_2021_WACV} on the socially sensitive attributes of gender, age, and race. In this evaluation, we plug FairFace as the bias assessment module and classify the generated images of Stable Diffusion 1.5, 2, and XL as well as real images from COCO and Flickr30k. We then compute the KL divergence between the predictions of the VQA and FairFace, by doing so we are assessing the agreement of the two models. This is shown in Table~\ref{tab:FairFace_eval_KL} and, as we can see, both models are highly aligned, proving the VQA model's robustness in both generative and real settings. We provide further quantitative evaluations of the VQA in the supplementary material.

==> sec_bak/3_method.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/method/Method_overview.pdf}
    \caption{Method.}
    \label{fig:method}
\end{figure*}

\section{Method}
In this section, we present our pipeline for proposing, assessing, and quantifying biases in generative models without the need to pre-define them. An overview is presented in Fig. \ref{fig:method}. We start from a dataset of real captions and we build, leveraging a LLM, a knowledge base of biases composed of specific information such as captions, questions, and classes all associated with the bias. This process allows us to create domain-specific knowledge, which may vary based on the dataset. In the second stage of our pipeline, the assigned captions for a particular bias are used to synthesize bias-specific images leveraging the target generative model. After generating the images, we leverage the knowledge base to assess and quantify the presence of each bias via Vision Question Answering (VQA) applied to the generated images. 

\subsection{Bias proposals}
In this section, we explain our \textit{bias proposals} module able to build the knowledge base $\knowledgebase$ of biases required to recognize and quantify them. This procedure leverages in-context learning, a well-known technique that consists of assigning to an LLM a specific task during inference, accompanied by specific instructions on how to perform it. In addition, a set of examples is given to the model to improve its performance similarly to existing works~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. Please see the supplementary material for further details about the system task and examples given to the LLM.

We start from a set of captions $\datasetcaptions$ provided by a real dataset. The LLM is explicitly tasked to provide knowledge about biases that may occur during the generation process if the specific captions are given to a generative model, thereby preventing the LLM from extracting biases inherent in the caption. Given a caption, we ask the LLM to output three main pieces of information: the bias name, a set of classes, and a question. The name allows us to identify the bias under study, and the set of classes and questions, allow us to recognize and quantify the bias at the third stage of our pipeline. To give a concrete example, if the caption is \textit{"A person running"} one of the proposed biases may be \textit{"person gender"}. In this case, the other pieces of information for this bias may be \textit{"Male"} and \textit{"Female"} as classes and \textit{"What is the gender of the person in the picture?"} as the question. 

More formally, given a caption $\singlecaption \in \datasetcaptions$, let the LLM's output be denoted as:
$$
    \text{LLM} \left ( \singlecaption \right )=\left (\biasname, \hat{\mathcal{C}} ,\hat{q}_t \right )
$$
where: $\biasname$ is the bias name, $\hat{C}$ is the set of associated classes, and $\hat{q}_t$ is the question assigned to the caption $\singlecaption$. We build the knowledge base $\knowledgebase$ by aggregating information for each bias where the bias names and classes are identical. We analyze in detail this post-processing procedure in the supplementary material. Thus, given a bias $\bias$, we define its knowledge base as:
$$
    \defineKB
$$
where: $\Tj$ is the set of captions assigned to $\bias$ and $\setquestions$ is the set of associated questions. We denote a piece of specific information as $\hat{\cdot}$ when entirely generated by the LLM. The information from the set of classes $\classes$ and $\setquestions$ will be used, in the third phase, as input to the VQA as a closed-form question to recognize the specific bias in the generated images. Executing this procedure on a set of captions builds a knowledge base of biases with specific information required to recognize them effectively.

The above-explained procedure can lead to undesirable consequences when a specific, bias-related characteristic is defined in the caption. For example, a sentence of the type \textit{"A man running"} should be avoided while studying gender-related biases as it explicitly specifies the attribute of the bias under study. To avoid this outcome, we apply a two-stage filtering: first, we ask the LLM to output whether the answer to the question $\singlequestion$ is embedded in the caption itself, if so the caption will not be considered for the specific bias $\bias$. Secondly, we leverage ConceptNET \cite{ConceptNET} to extract synonyms of the classes $\classes$ for the specific bias $\bias$, then we filter the captions containing such synonyms. The first stage is required since LLM knows the context of the caption, and synonyms may not capture the whole picture. On the other hand, the second stage ensures that specific words related to the bias are not present in the caption improving the robustness of the pipeline.

By executing the above framework we produce bias proposals that will be assessed in the next stages of our pipeline.

\subsection{Bias assessment and quantification}
At this stage, we aim to assess the presence of each previously proposed bias. We employ the target generative model G to produce a synthetic dataset using the set of captions $\Tj \subseteq \datasetcaptions$ associated with the bias $\bias$. This process results in a set of images for each bias. The assessment of biases is conducted via Vision Question Answering. For each bias $\bias$, we utilize a state-of-the-art VQA model on the generated images, answering the associated questions $\setquestions$ in a closed form by providing the model with answer choices resembling the classes $\classes$. This approach enables statistical analyses by exploring the distribution over the classes. During this phase, we consider the context of each caption by building the generated dataset with $N$ images for every caption. This consideration of context is essential for comprehensive bias evaluation. This framework provides the basis for studying the bias in a contextualized or context-free form.

\subsubsection{Contextualize bias}
In the contextualized formulation, we are interested in capturing the bias $\bias$ considering the context of the caption. For instance, let's suppose we possess two captions of the form \textit{"A military person is running"} and \textit{"A person is running"}, they are both agnostic to the bias \textit{"person gender"}, but the bias direction and magnitude may vary depending on the context, thus, to take the context into account we generate $N$ images for each caption $\singlecaption \in \Tj$. We define this set of images as $\defineI$ and the expected probability over the classes $\classes$ condition on context $t$ as:
$$
    \definePcontext
$$
where: $\indicatorfunction$ denotes the indicator function that is $1$ when $c$ is equal to the output of the $VQA$ model applied to the generated image $I_z$, and $0$ otherwise and $\hat{q}_t$ is the question assigned to $t$ from the previous phase. This formulation allows us to study how the bias $\bias$ varies in relation to the context of each caption $t$.

\subsubsection{Context-free bias}
In this approach, we are interested in understanding the behavior of the target generative model without considering the context. This is significant as it allows us to study the scale of the impact of context on the given bias and facilitates the study of the model in a more general setting. Concretely, given a bias $\bias$, we define its synthetic dataset as $\definesyntheticdataset$, that is we consider the whole dataset of generated images regardless of the caption context. In this scenario, we compute the context-free expected probability distribution over the classes $\classes$ as:
$$
    \definePfreecontext
$$


\subsubsection{Bias quantification and ranking}
The open-set nature of our setting challenges the study and understanding of the multiple biases. We address this issue by ranking the biases based on their intensity. We use the entropy computed over the categorical distributions defined above. Since we are required to compare these values across different distributions, we use the normalized entropy $\mathcal{H}$ \cite{wilcox1967indices}. In order to make the entropy more human-readable we define the intensity of a bias $\bias$ as $1-\mathcal{H}$. The intensity is bounded in $[0,1]$ where $0$ describes high uncertainty over the classes and thus low bias, instead $1$ expresses low uncertainty thus high bias. We apply this formulation over the contextualized bias and context-free bias defined above. When applied to the contextualized distribution we average over all the captions $\Tj$. This formulation allows us to rank the found biases by bias intensity.




% We task the LLM leveraging in-context learning, a well-known technique that consists of assigning to the LLM a specific task during inference, accompanied by specific instructions on how to perform it. 



% In addition, a set of examples is given to the model to improve its performance similarly to existing works~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. We ask the LLM to output a set of biases for each caption alongside a set of classes and a question for each identified bias. By doing so we build a knowledge base of biases which are specific for each caption, comprising a set of classes and questions. Afterward, we sample $N$ captions for each bias and we generate $K$ images for each caption, in this way we make sure that if the bias is present it does not depend from the caption. This process generates $N\times K$ images for each bias. The third and final stage exploits a Vision Question Answering model which is applied to the generated images and, for each bias, we ask the model to answer the bias specific question given by the LLM in a closed form by providing the classes. We quantify the presence of the biases by applying two metrics to the extracted class distributions: Entropy and KL divergence. 


% To be added in the method section:

% We first perform in-context learning on a LLM which is a well-known zero-shot method. In-context learning assigns to the LLM a specific task during inference, accompanied by specific instructions on how to perform it, and, in addition, a set of examples is given to the model to improve its performance~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}. 
% Our pipeline is composed of three main stages: bias identification, image generation and bias recognition. In the first stage, we task a LLM to identify a set of possible biases that may occur during the generation process given a set of captions. By doing so we identify the set of biases that are going to be studied 
% In our pipeline, we make use of in-context learning. This method assigns to the LLM a specific task during inference, accompanied by specific instructions on how to perform it, and, in addition, a set of examples is given to the model to improve its performance~\cite{TIFA_2023_ICCV, NEURIPS2020_gpt_3_few_shot, ICLR_2023_selective_annotations}.

% we exploit the recent advancements in foundation models~\cite{NEURIPS2020_gpt_3_few_shot, NEURIPS2022_Chain_of_Thougth, li2023blip2, liu2023llava, liu2023improvedllava}. 

==> sec_bak/4_results.tex <==
\input{images/comparison/xl_2_coco}
\section{Experiments}
In this section, we present the results and evaluations of the proposed pipeline by detecting biases on three diffusion-based generative models: Stable diffusion XL~\cite{podell2023sdxl}, 2~\cite{LDM_2022_CVPR}, and 1.5~\cite{LDM_2022_CVPR}. Existing works on bias mitigation in generative models~\TODO{cite} commonly rely on a classifier on the specific bias to detect, thus we compare the proposed pipeline with a SOTA classifier on socially sensitive biases showing its alignment with the classifier's outcome. We run a thorough evaluation of each component showing its robustness in bias detection settings. Finally, we show that the same pipeline can be applied to real datasets.  and, by employing an image captioner, to unconditional generative models and image-only datasets.

In this section, we present a set of experiments to quantitatively and qualitatively evaluate the proposed pipeline.  

\subsection{Pipeline Implementation}
\paragraph{Implementation details} We use LLama2-7B as LLM and, since the VQA model is crucial in recognizing biases in our pipeline, we test multiple SOTA VQA models. The evaluation of these models on the setting of bias detection highlights LLava2-13B~\cite{liu2023llava, liu2023improvedllava} as the most robust model, consequently, we employ it as the VQA model in our pipeline. This analysis is available in the supplementary material. We note that the proposed framework is highly flexible allowing the changing of LLM and VQA as needed. This flexibility facilitates the incorporation of future advancements and the fulfillment of specific requirements if needed. One of the goals of this work is to assess biases in the context of real-life usage of generative models. In a practical scenario, a user using open-source generative models typically generates a set of images for quick and human-readable selection. Considering this practical scenario and the high volume of images to be generated in our setting, we set the number of generated images per caption to $N=10$. In our experiments, we leverage $100$ prompts for each bias effectively generating $1000$ images for each proposed bias. 

\paragraph{Dataset} We leverage captions from the real datasets COCO~\cite{DBLP:journals/corr/LinMBHPRDZ14}, Flickr30k~\cite{young-etal-2014-image}, and open images~\cite{DBLP:journals/corr/abs-1811-00982}. COCO~\cite{DBLP:journals/corr/LinMBHPRDZ14} is a large-scale dataset for segmentation, object detection, and captioning. It is composed of over $123$K images with $5$ captions for each image. While using this dataset, we use captions assigned to images portraying a single person. This choice aims to enable our pipeline to focus on identifying socially sensitive biases. However, despite this primary focus, we show that our pipeline can likewise detect object-related biases. Similarly, Flickr30k~\cite{young-etal-2014-image} comprises $30$K with $5$ caption per image. In this case, we use the whole set of cations. Open images~\cite{DBLP:journals/corr/abs-1811-00982} is a large-scale collection of $~9$M images and annotations for object detection, segmentation, action recognition, and localization. Since the original dataset does not provide captions, we use the $n-captions$ captions provided by the localized narratives~\cite{PontTuset_eccv2020}. 
% Finally, we employ FFHQ~\cite{Karras_2019_CVPR} as the image-only dataset featuring $70$K facial images.

\input{images/qualitatives/qualitatives_new_biases}
\input{images/qualitatives/qualitatives_person_novel_biases}
\input{images/qualitatives/qualitatives_person}
\subsection{Qualitative results}
In this section, we discuss the qualitative results of the proposed method applied on Stable Diffusion XL~\cite{podell2023sdxl}. It is essential to consider biases discovered by both context-free and contextualized approaches. In the former case, we focus on the broader perspective providing insights into the prevalence and direction of the various biases. Meanwhile, in the latter case, we delve into a more granular understanding of biases highlighting the importance of the context in influencing the specific direction of biases. For this reason, we analyze the results at the context level to assess the contextualized bias in comparison to the free setting. 

In contrast to conventional biases explored in existing works~\TODO{cite} (e.g., person gender, person race, etc.), we show, in Figure~\ref{fig:qualitatives_others}, novel biases discovered by the proposed method. The results show how the pipeline successfully identifies biases related to objects and animals. In the context-free formulation, the identified direction of the bias for \textit{``train color"} and \textit{``laptop brand"} is \textit{``yellow"} and \textit{``Apple"} respectively. This correlation is consistently validated at the context level as depicted in the figure. A parallel observation occurs with \textit{``horse breed} where the bias direction is consistently identified as \textit{``quarter horse"} in both settings. 

While exploring new biases, we keep a crucial focus on socially sensitive biases. Consequently, in Figure~\ref{fig:qualitatives_novel_person}, we provide qualitative results on biases related to individuals while varying from the traditional person-related biases typically examined in the literature~\TODO{cite}. Figure~\ref{fig:qualitatives_novel_person} shows two child-related and one person-related biases. In the former case, the pipeline discovers that \textit{``gender"} and \textit{``race"} prejudices, similarly to person-related biases, are likewise present in the child domain. In the latter, we show \textit{``attire"} as a novel bias within the person domain. These cases highlight the importance of exploring biases at the contextual level for a more comprehensive analysis. Naturally, the context-level direction of the biases does not always align with the context-free scenario. While there may be a clear bias direction on average across all generated images, this may not be true in every single context, emphasizing the importance of considering context-level biases. We demonstrate this in Figure~\ref{fig:qualitatives_novel_person} on \textit{``child gender"} where the bias leans towards \textit{``male"}, contrary to the context-free bias direction of \textit{``female"}. Likewise, the global bias direction for \textit{``person attire"} is \textit{``casual"}, yet in this context instance, it is \textit{``formal"}. 

Referring to Figure~\ref{fig:qualitatives_novel_person}, it is important to pause on the example of \textit{``child race"}. Here, the context-free direction of the bias is \textit{``caucasian"} following the conventional person race bias towards the white people~\TODO{cite}. Instead, in this specific instance, the generative model consistently associates a black child with a poor setting which is highly undesirable. This connection between racial identity and socioeconomic status in the context of a "dirty road" reinforces harmful stereotypes and proves the need to consider novel biases within bias mitigation frameworks.

In addition to addressing novel biases, it is critical to comprehend the performance of the proposed method against conventional biases. In Figure~\ref{fig:qualitatives_person}, we present three well-known biases identified by the pipeline. While \textit{``person gender"} and \textit{``person age"} follow the biased direction of the context-free formulation, represented by \textit{``Male"} and \textit{``Middle-aged"}, it is essential to highlight, once more, the importance of the context. For instance, in person race, we observe that a seemingly neutral and agnostic caption can result in significant stereotyping.

This double approach of context-free and contextualized biases ensures a thorough comprehension of emerging biases in both novel and socially significant contexts. The results we have shown emphasize the necessity for more inclusive open-set bias detection frameworks. We provide additional qualitative results and model-level comparisons in the supplementary material.


==> sec_template/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec_template/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec_template/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec_template/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/CFD_eval.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
        \toprule
        \textbf{Attribute} & Accuracy & F1 \\
        \midrule
         Gender & 97.89 & 97.92 \\
         Race & 77.60 & 72.98 \\
        \bottomrule
    \end{tabular}
    \caption{Self-identification evaluation.}
    \label{tab:VQA_eval_coco}
\end{table}

==> tables/KL_div_fairface_ffhq_eval.tex <==
\begin{table}[h!]
    \begin{tabular}{ccccc}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{ffhq}              \\
                            & gender  & age     & race 7  & race 4  \\ \hline
    original                & 0.00066 & 0.00043 & 0.90241 & 0.00779 \\
    stylegan3               & 0.00548 & 0.00191 & 0.95730 & 0.02328 \\ \hline
    \end{tabular}
    \caption{ffhq}
    \label{tab:my-table} 
\end{table}

==> tables/LLM_eval.tex <==
% \begin{table}[t]
%     \centering
%     \begin{tabular}{l|cccc}
%     \toprule
%     \textbf{Dataset}  & \textbf{Top-1}  & \textbf{Top-2}  & \textbf{Top-3}  & \textbf{Top-4 } \\ \midrule
%     StereoSet~\cite{nadeem2020stereoset}        & 60.39  & 87.02  & 90.85  & -      \\
%     Crows~\cite{nangia2020crows}                & 61.43  & 78.03  & 82.96  & 86.50 \\ \bottomrule
%     \end{tabular}
%     \caption{Accuracy of LLama2-7B in stereotype detection on the StereoSet and Crows datasets.}
%     \label{tab:LLM_eval}
% \end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{l|cccc}
    \toprule
    \textbf{Dataset}  & \textbf{Top-1}  & \textbf{Top-2}  & \textbf{Top-3} \\ \midrule
    Crows~\cite{nangia2020crows}                & 65.43  & 80.59  & 82.48  \\ 
    StereoSet~\cite{nadeem2020stereoset}        & 52.00  & 65.05  & 72.76  \\ \bottomrule
    \end{tabular}
    \caption{Accuracy of LLama2-7B in stereotype detection on the StereoSet and Crows datasets.}
    \label{tab:LLM_eval}
\end{table}

==> tables/vqa_eval_coco.tex <==
% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{ccccccccc}
%         \hline
%         \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Gender} & \multicolumn{2}{c|}{Age} & \multicolumn{2}{c|}{Race 4 classes} & \multicolumn{2}{c|}{Race 7 classes} \\ 
%                                & Accuracy & f1-score & Accuracy & f1-score & Accuracy & f1-score & Accuracy & f1-score \\
%         \hline
%          llava-1.5-13b     & 92.83          & \textbf{83.21}    & \textbf{72.27}    & \textbf{70.00}    & \textbf{55.91}    & \textbf{44.33}    & 47.83             & 28.06 \\
%          clip-vit          & 87.25          & 54.45             & 42.51             & 33.79             & 29.33             & 23.73             & 18.90             & 17.09 \\
%          promptcap-t5large & 90.24          & 79.54             & 42.14             & 31.61             & 52.36             & 35.64             & 46.26             & 21.10 \\
%          llava-1.5-7b      & 92.03          & 82.33             & 66.54             & 62.16             & 55.71             & 42.80             & \textbf{48.82}    & \textbf{31.53} \\
%          clip-L            & 91.43          & 75.46             & 58.96             & 45.77             & 36.02             & 33.60             & 16.54             & 15.32 \\
%          ofa-large         & \textbf{93.03} & 83.07             & 53.79             & 41.72             & 24.61             & 21.22             & 37.60             & 15.15 \\
%          vilt              & 85.26          & 73.03             & 42.70             & 20.00             & 44.49             & 29.01             & 37.01             & 15.42 \\
%          mplug-large       & \textbf{93.03} & 82.81             & 61.37             & 52.74             & 21.46             & 23.26             & 43.31             & 19.79 \\
%          open-clip-vit     & 78.88          & 67.63             & 20.89             & 20.80             & 37.20             & 33.37             & 14.17             & 13.79 \\
%          blip-large        & 92.23          & 82.18             & 48.61             & 31.29             & 36.22             & 35.52             & 47.83             & 25.73 \\
%          git-large         & 92.03          & 81.60             & 44.55             & 24.47             & 43.70             & 34.21             & 46.65             & 22.81 \\
%          blip2-flant5xxl   & 90.64          & 80.14             & 62.85             & 61.46             & 37.80             & 37.91             & 14.37             & 13.26 \\
%         \hline
%     \end{tabular}
%     \caption{VQA evaluation on the generated images using coco captions}
%     \label{tab:VQA_eval_coco}
% \end{table*}

\begin{table}
    \centering
    \begin{tabular}{lcccccc}
        \midrule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Gender}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c}{\textbf{Race}} \\ \cmidrule{2-7}
                               & Acc & \multicolumn{1}{c|}{F1} & Acc & \multicolumn{1}{c|}{F1} & Acc & \multicolumn{1}{c}{F1} \\
        \midrule
         clip-vit          & 87.25          & 54.45             & 42.51             & 33.79             & 29.33             & 23.73             \\
         promptcap-t5large & 90.24          & 79.54             & 42.14             & 31.61             & 52.36             & 35.64             \\
         llava-1.5-7b      & 92.03          & 82.33             & 66.54             & 62.16             & 55.71             & 42.80             \\
         clip-L            & 91.43          & 75.46             & 58.96             & 45.77             & 36.02             & 33.60             \\
         ofa-large         & \textbf{93.03} & 83.07             & 53.79             & 41.72             & 24.61             & 21.22             \\
         vilt              & 85.26          & 73.03             & 42.70             & 20.00             & 44.49             & 29.01             \\
         mplug-large       & \textbf{93.03} & 82.81             & 61.37             & 52.74             & 21.46             & 23.26             \\
         open-clip-vit     & 78.88          & 67.63             & 20.89             & 20.80             & 37.20             & 33.37             \\
         blip-large        & 92.23          & 82.18             & 48.61             & 31.29             & 36.22             & 35.52             \\
         git-large         & 92.03          & 81.60             & 44.55             & 24.47             & 43.70             & 34.21             \\
         blip2-flant5xxl   & 90.64          & 80.14             & 62.85             & 61.46             & 37.80             & 37.91             \\
         \rowcolor{gray!20} llava-1.5-13b     & 92.83          & \textbf{83.21}    & \textbf{72.27}    & \textbf{70.00}    & \textbf{55.91}    & \textbf{44.33}    \\
        \midrule
    \end{tabular}
    \caption{VQA evaluation on the generated images using coco captions}
    \label{tab:VQA_eval_coco}
\end{table}

==> tables/vqa_eval_flickr_30k.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcccccccc}
        \midrule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Gender}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c}{\textbf{Race}} \\ \cmidrule{2-7}
                               & Acc & \multicolumn{1}{c|}{F1} & Acc & \multicolumn{1}{c|}{F1} & Acc & F1 \\
        \midrule
         clip-vit          & 90.89          & 66.89             & 56.31             & 48.60             & 26.62             & 25.07             \\
         promptcap-t5large & 89.21          & 71.13             & 46.46             & 32.82             & 50.72             & 35.19             \\
         llava-1.5-7b      & 89.93          & 72.20             & 71.46             & 57.48             & 57.91             & 45.00             \\
         clip-L            & 91.61          & 70.80             & 65.66             & 52.11             & 37.05             & 36.97             \\
         ofa-large         & 91.37          & 73.31             & 61.11             & 40.56             & 28.06             & 24.39             \\
         vilt              & 82.25          & 64.48             & 45.71             & 23.84             & 45.68             & 28.32             \\
         mplug-large       & \textbf{91.85} & 73.49             & 71.72             & 58.89             & 25.90             & 25.82             \\
         open-clip-vit     & 79.86          & 63.95             & 31.31             & 30.48             & 43.88             & 40.35             \\
         blip-large        & 91.61          & \textbf{73.73}    & 47.73             & 30.72             & 34.89             & 31.31             \\
         git-large         & 91.37           & 73.31             & 42.93             & 22.62             & 47.84             & 40.71             \\
         blip2-flant5xxl   & 89.93          & 71.60             & 70.71             & 59.82             & 35.97             & 37.55             \\
         \rowcolor{gray!20} llava-1.5-13b     & 90.89          & 73.13             & \textbf{74.75}    & \textbf{65.52}    & \textbf{58.27}    & \textbf{48.05}    \\
        \midrule
    \end{tabular}
    \caption{VQA evaluation on the generated images using flickr30k captions}
    \label{tab:VQA_eval_flickr30k}
\end{table} 
